Quadcopter Tracking Using Euler-Angle-Free Flatness-Based Control

Quadcopter trajectory tracking control has been extensively investigated and implemented in the past. Available controls mostly use the Euler angle standards to describe the quadcopters rotational kinematics and dynamics. As a result, the same rotation can be translated into different roll, pitch, and yaw angles because there are multiple Euler angle standards for characterization of rotation in a 3-dimensional motion space. Additionally, it is computationally expensive to convert a quadcopters orientation to the associated roll, pitch, and yaw angles, which may make it difficult to track quick and aggressive trajectories. To address these issues, this paper will develop a flatness-based trajectory tracking control without using Euler angles. We assess and test the proposed controls performance in the Gazebo simulation environment and contrast its functionality with the existing Mellinger controller, which has been widely adopted by the robotics and unmanned aerial system (UAS) communities.

==> preliminaries-hossein.tex <==
\section{QUADCOPTER MODEL}
\label{sec:model}

% \subsection{Quadcopter dynamics}

% We denote the inertial reference frame with base vectors $\left(\vu{i}, \vu{j}, \vu{k}\right)$ and the quadcopter's local frame with $\left(\vu{i}_B, \vu{j}_B, \vu{k}_B\right)$.

% We define the quadcopter's state $\boldsymbol{s}$ as:
% \begin{equation}
%     \boldsymbol{s} = \begin{bmatrix}\boldsymbol{r}& \dot{\boldsymbol{r}}& \boldsymbol{R}&\boldsymbol{\omega}\end{bmatrix}.
% \end{equation}
% where $\boldsymbol{r}$ is its position, $\boldsymbol{R}$ is its orientation described with a rotation matrix, and $\boldsymbol{\omega}$ is its angular velocity.

% $\boldsymbol{R}$ and its derivative can be expressed as:
% \begin{subequations}
% \begin{equation}
%     \boldsymbol{R} = \begin{bmatrix}
%     \vu{i}_B& \vu{j}_B& \vu{k}_B
%     \end{bmatrix},
% \end{equation}
% \begin{equation}
%     \dot{\boldsymbol{R}} = \begin{bmatrix}
%     \boldsymbol{\omega} \times \vu{i}_B& \boldsymbol{\omega} \times \vu{j}_B& \boldsymbol{\omega} \times \vu{k}_B
%     \end{bmatrix}.
% \end{equation}
% \end{subequations}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=3in]{figures/formation.png}
% \caption{Quadcopter reference pose. Red arrows show the rotation direction of each rotor.}
% \label{fig:reference_frame}
% \end{figure}

\begin{figure}
 \centering
 \subfigure[]{\includegraphics[width=0.43\linewidth]{figures/formation.png}}
  \subfigure[]{\includegraphics[width=0.55\linewidth]{figures/heading_pic.png}}
%  \subfigure[]{\includegraphics[width=0.32\linewidth]{Example-Initial-Formation.png}}
%  \subfigure[]{\includegraphics[width=0.32\linewidth]{Example-Final-FormationAI.png}}
%   \subfigure[$\varpi_{i,2}~\forall i\in \mathcal{V}$]{\includegraphics[width=0.9\linewidth]{SecondAngularSpeeds-V2.png}}
%   \subfigure[$\varpi_{i,3}~\forall i\in \mathcal{V}$]{\includegraphics[width=0.9\linewidth]{ThirdAngularSpeeds-V2.png}}
%   \subfigure[$\varpi_{i,3}~\forall i\in \mathcal{V}$]{\includegraphics[width=0.9\linewidth]{FourthAngularSpeeds-V2.png}}
%   \subfigure[$t=100s$]{\includegraphics[width=0.24\linewidth]{t100.jpg}}
%   \subfigure[$t=200s$]{\includegraphics[width=0.24\linewidth]{t{\color{black}400}.jpg}}
%   \subfigure[$t=400s$]{\includegraphics[width=0.24\linewidth]{t400.jpg}}
%   \subfigure[$t=500s$]{\includegraphics[width=0.24\linewidth]{t500.jpg}}
%   \subfigure[$t=650s$]{\includegraphics[width=0.24\linewidth]{t650.jpg}}
%   \subfigure[$t=812s$]{\includegraphics[width=0.24\linewidth]{t812.jpg}}
\vspace{-0.3cm}
     \caption{(a)  Quadcopter reference pose. Red arrows show the rotation direction of each rotor. (b) Heading vector and heading constraints visualized {\color{red}You did not use $\hat{x}_b,\hat{y}_b,\hat{z}_b$ in the text}.}
\label{fig:reference_frame}
\end{figure}
The quadcopter has a mass $m$ and a diagonal inertia matrix $\boldsymbol{J}$ with entries $\left(J_x, J_y, J_z\right)$. It is setup in a ``+'' formation with a distance from rotors to center of mass $L$ as shown in Fig. \ref{fig:reference_frame} (a). The $i$-th rotor spins at angular speed $s_i \in \left[0, s_{max}\right]$ where $s_{max}$ is the maximum rotor angular speed which is the same for every rotor $i\in \left\{1,\cdots,4\right\}$. The $i$-th rotor creates a thrust $p_i = k_F s_i^2$ and a torque $\tau_i = \pm k_M s_i^2$ both in the $\vu{k}_B$ direction where $k_F$ and $k_M$ are aerodynamic constants. Collectively, they create a net thrust force $p \vu{k}_B$ and net torque $\boldsymbol{\tau}$ given by:
\begin{equation}
\label{eq:rotors}
    \begin{bmatrix}
    p\\
    \boldsymbol{R}^T\boldsymbol{\tau}\\
    \end{bmatrix}
    =
    \begin{bmatrix}
    k_F&k_F&k_F&k_F\\
    0&-k_FL&0&k_FL\\
    -k_FL&0&k_FL&0\\
    -k_M&k_M&-k_M&k_M
    \end{bmatrix}
    \begin{bmatrix}
    s_{1}^2\\
    s_{2}^2\\
    s_{3}^2\\
    s_{4}^2\\
    \end{bmatrix}.
\end{equation}
By applying the Newton's Second law, the transnational and rotational dynamics of the quadcopter is given by
\begin{subequations}
\begin{equation}
\label{eq:translation}
    m \ddot{\boldsymbol{r}} = p\vu{k}_B - mg\vu{k},
\end{equation}
\begin{equation}
\label{eq:rotational}
    \boldsymbol{J}\boldsymbol{\alpha} + \boldsymbol{\omega}\times \left(\boldsymbol{J}\boldsymbol{\omega}\right) = \boldsymbol{\tau},
\end{equation}
\end{subequations}
where $\boldsymbol{\alpha} = \dot{\boldsymbol{\omega}}$ is the quadcopter's angular acceleration. 
We denote the inertial reference frame with base vectors $\left(\vu{i}, \vu{j}, \vu{k}\right)$ and the quadcopter's local frame with $\left(\vu{i}_B, \vu{j}_B, \vu{k}_B\right)$. Next, we overview the Snap and Mellinger trajectory control in Subsections \ref{Snap Control} and \ref{Mellinger Control}.

\subsection{Snap Control}\label{Snap Control}
For the Snap control, the motion of the quadcopter is modeled by \cite{Snap}
\begin{equation}
\label{generalnonlineardynamics}
\begin{cases}
    \dot{\mathbf{x}}=\mathbf{f}\left(\mathbf{x}\right)+\mathbf{g}\mathbf{u}\\
    \mathbf{y}=\begin{bmatrix}
    x&y&z&\psi
    \end{bmatrix}^T
    \end{cases}
    ,
\end{equation}
where $\mathbf{y}$ is the output vector, $\mathbf{f}\in \mathbb{R}^{14\times 1}$ and $\mathbf{g}\in \mathbb{R}^{14\times4}$ are smooth functions defined in \cite{Snap}, and 
\begin{subequations}
%\vspace{-0.2cm}
\begin{equation}
% \resizebox{0.99\hsize}{!}{%
% $
    \mathbf{x}=[
x~y~z~\dot{x}~\dot{y}~\dot{z}~\phi~\theta~\psi~\dot{\phi}~\dot{\theta}~\dot{\psi}~p~\dot{p}
]
^T,
% $
% }
\end{equation}
%\vspace{-0.2cm}
\begin{equation}
% \resizebox{0.99\hsize}{!}{%
% $
    \mathbf{u}=\begin{bmatrix}
\ddot{p}&\boldsymbol{\tau}^T
\end{bmatrix}
% ^T=\begin{bmatrix}
% \ddot{p}&\ddot{\phi}&\ddot{\theta}&\ddot{\psi}
% \end{bmatrix}^T,
% $
% }
\end{equation}
\end{subequations}
are the state vector and the control input of the quadcopter, respectively ($x$, $y$, and $z$ are position components, $\phi$, $\theta$, $\psi$ are the roll, pitch, and yaw angles, and $p$ is the thrust force magnitude).
% In \eqref{generalnonlineardynamics},
% \begin{subequations}
% %\vspace{-0.2cm}
% \begin{equation}
% \mathbf{f}\left(\mathbf{x}\right)=\begin{bmatrix}\dot{x}&
%     \dot{y}&
%     \dot{z}&
%     \left({\frac{p}{m}\hat{\mathbf{b}}_3-{g}\hat{\mathbf{e}}_3}\right)^T&
%     % \frac{p}{m}\left(\sin{\phi}\sin{\psi} + \cos{\phi}\cos{\psi}\sin{\theta}\right)&
%     % \frac{p}{m}\left(\cos{\phi}\sin{\psi}\sin{\theta}- \sin{\phi}\cos{\psi}\right)&
%     % \frac{p}{m}\cos{\phi}\cos{\theta}-9.81&
%     \dot{\phi}&
%     \dot{\theta}&
%     \dot{\psi}&
%     0&
%     0&
%     0&
%     \dot{p}&
%     0
%     % {\dot{p}\over m}\left(\sin{\phi}\sin{\psi} + \cos{\phi}\cos{\psi}\sin{\theta}\right)+\frac{p}{m}\left[-\dot{\phi}\left(\cos{\psi} \sin{\phi} \sin{\theta} - \cos{\phi}\sin{\psi}\right)\right]\\
%     % {\dot{p}_i\over m}\left(\cos{\phi}\sin{\psi}\sin{\theta}- \sin{\phi}\cos{\psi}\right)+{p_i\over m}\left[-\dot{\phi}_i\left(\cos{\phi}\cos{\psi} +\sin{\phi}\sin{\psi}\sin{\theta}\right)\right]\\
%     % {\dot{p}_i\over m}\cos{\phi}\cos{\theta}+{p_i\over m}\left[-\dot{\phi}_i\cos{\theta}\sin{\phi}\right]\\
%     \end{bmatrix}^T
% %     \mathbf{f}\left(\mathbf{x}_i\right)=\begin{bmatrix}
% % \dot{\mathbf{r}}_i\\
% % -g\hat{\mathbf{e}}_3\\
% % \mathbf{\Gamma}_i^{-1}\left(\phi,\theta,\psi\right){\color{black}\bf{\omega}}_i\\
% % -\mathbf{J}_i^{-1}\left({\color{black}\bf{\omega}}_i\times \left(\mathbf{J}_i{\color{black}\bf{\omega}}_i\right)\right)\\
% % \dot{p}_i\\
% % 0\\
% % \end{bmatrix}+\begin{bmatrix}
% % \mathbf{0}_{3\times 1}\\
% % {p_i\over m}\hat{\mathbf{k}}_{b,i}\\
% % \mathbf{0}_{8\times 1}\\
% % \end{bmatrix}
% % \begin{bmatrix}
% % \dot{\mathbf{r}}_i\\
% % \frac{1}{m}p_i\hat{\mathbf{k}}_{b,i}-g\hat{\mathbf{e}}_3\\
% % \mathbf{\Gamma}_i^{-1}\left(\phi,\theta,\psi\right){\color{black}\bf{\omega}}_i\\
% % \mathbf{J}_i^{-1}{\color{black}\bf{\omega}}_i\times \left(\mathbf{J}_i{\color{black}\bf{\omega}}_i\right)\\
% % \dot{p}_i\\
% % 0
% % \end{bmatrix}
% ,
% \end{equation}
% %\vspace{-0.2cm}
% \begin{equation}
%     \mathbf{G}=
%     % \begin{bmatrix}
%     % {\mathbf{g}}_1&{\mathbf{g}}_2&{\mathbf{g}}_3&{\mathbf{g}}_4
%     % \end{bmatrix}
% \begin{bmatrix}
% \mathbf{0}_{9\times 1}&\mathbf{0}_{9\times 3}\\
% \mathbf{0}_{3\times 1}&\mathbf{I}_3\\
% 0&\mathbf{0}_{1\times 3}\\
% 1&\mathbf{0}_{1\times 3}\\
% \end{bmatrix}
% ,
% \end{equation}
% \end{subequations}
% are smooth functions obtained in Ref. \cite{rastgoftar2021safe}, where
% $\mathbf{I}_3\in \mathbb{R}^{3\times 3}$ is the identity matrix, $\mathbf{0}_{3\times 1}\in \mathbb{R}^{3\times 1}$, $\mathbf{0}_{3\times 3}\in \mathbb{R}^{3\times {3}}${, and $\mathbf{0}_{3\times 9}\in \mathbb{R}^{3\times {9}}$} are the zero-entry matrices.
We use the input-state feedback linearization approach, presented in \cite{Snap}, for low-level trajectory tracking. To this end, we use state transformation 
\[
\mathbf{z}=\left[{\boldsymbol{r}}~\dot{\boldsymbol{r}}~\ddot{\boldsymbol{r}}~\dddot{\boldsymbol{r}}~\psi~\dot{\psi}\right]
\] 
to convert the quadcopter state $\mathbf{x}$ to the state of the external dynamics $\mathbf{z}$, where the external dynamics is given by \cite{Snap}
\begin{subequations}
\begin{equation}
\begin{split}
    \ddddot{\boldsymbol{r}} = \ & - \boldsymbol{K}_1 \left(\dddot{\boldsymbol{r}} - \dddot{\boldsymbol{r}}_T\right) - \boldsymbol{K}_2 \left(\ddot{\boldsymbol{r}} - \ddot{\boldsymbol{r}}_T\right) \\ - & \boldsymbol{K}_3 \left(\dot{\boldsymbol{r}} - \dot{\boldsymbol{r}}_T\right) - \boldsymbol{K}_4 \left(\boldsymbol{r} - \boldsymbol{r}_T\right),
\end{split}
\end{equation}
\begin{equation}
\label{psidynamics}
    \ddot{\psi} = - K_5 \left(\dot{\psi} - \dot{\psi}_T\right) - K_6 \left(\psi - \psi_T\right),
\end{equation}
\end{subequations}
where $\boldsymbol{r}_T(t)$ and $\psi_T(t)$ are the desired trajectory and yaw angle of the quadcopter, where 
\[
\boldsymbol{s}=\left(\boldsymbol{r}~\dot{\boldsymbol{r}}~\ddot{\boldsymbol{r}}~\dddot{\boldsymbol{r}}~\boldsymbol{R}~\boldsymbol{\omega}\right)
\]
aggregates the quadcopter sensor measurements. Note that $\boldsymbol{r}$, $\dot{\boldsymbol{r}}$, $\ddot{\boldsymbol{r}}$, and $\dddot{\boldsymbol{r}}$ are measured the motion capture system, and quadcopter orientation, specified by rotation matrix $\boldsymbol{R}=\left[\vu{i}_B~\vu{j}_B~\vu{k}_B\right]$, and angular velocity $\boldsymbol{\omega}$ are measured by the on-board sensor of a quadcopter.

In \cite{Snap}, we relied on Euler angles to control the quadcopter, specifically for dynamics \eqref{psidynamics}, which requires knowing  actual $\psi$ and $\dot{\psi}$. Indeed, by knowing sensory information $\boldsymbol{R}$ and $\boldsymbol{\omega}$, we can determine ${\psi}$ and $\dot{\psi}$ but at significant computation cost. Additionally,  Euler angular standards used by physics-based simulation software are not the same, therefore, different values of Euler angles are obtained for the same rotation matrix $\boldsymbol{R}$.

This paper overcomes the above issues by obtaining $\psi$, $\dot{\psi}$, $\boldsymbol{\tau}$, and thrust force $p$ without using the Euler angles only based on the sensor information $\mathbf{s}=\left(\boldsymbol{r}~\dot{\boldsymbol{r}}~\ddot{\boldsymbol{r}}~\dddot{\boldsymbol{r}}~\boldsymbol{R}~\boldsymbol{\omega}\right)$.
% \begin{equation}
% \mathbf{z}(\mathbf{x})=\begin{bmatrix}x&y&z&\dot{x}&\dot{y}&\dot{z}&\ddot{x}&\ddot{y}&\ddot{z}&\dddot{x}&\dddot{y}&\dddot{z}&\psi&\dot{\psi}\end{bmatrix}^T.
% \end{equation}

\subsection{Mellinger Control}\label{Mellinger Control}

\subsection{Heading model}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=3in]{figures/heading_pic.png}
% \caption{Heading vector and heading constraints visualized.}
% \label{fig:heading_pic}
% \end{figure}

In flight, the quadcopter tries to track a trajectory position $\boldsymbol{r}_T$ and a trajectory yaw $\psi_T$. Yaw is related to the  heading vector
$\vu{h}$ by
\begin{equation}
\label{eq:heading}
    \vu{h} = \cos(\psi)\vu{i} + \sin(\psi)\vu{j}.
\end{equation}
From Eq. \eqref{eq:translation}, we also obtain 
\begin{equation}
      \vu{k}_B={m \ddot{\boldsymbol{r}}+ mg\vu{k}\over p},
\end{equation}
{\color{blue}We use the $3-2-1$ Euler angle standard to characterize rotation of the quadcopter by roll angle $\phi$, pitch angle $\theta$, and yaw angle $\psi$. 
% \begin{proposition}
% Under the $3-2-1$ Euler angle standard, for characterizing rotation,  
% \end{proposition}
We constrain that the pitch angle $\theta$ (the second Euler angle) to satisfy $\left|\theta\right|<90$. Then, }
the heading vector $\vu{h}$ satisfies the 
\begin{subequations}
\begin{equation}
\label{eq:heading_constraint_1}
    \left(\vu{k} \times \vu{h}\right).\vu{i}_B = 0,
\end{equation}
\begin{equation}
\label{eq:heading_constraint_2}
    \vu{h}.\vu{i}_B > 0.
\end{equation}
\end{subequations}

% Note that the proofs for constraints \eqref{eq:heading_constraint_1} and \eqref{eq:heading_constraint_2} are provided in the Appendix.
% constraints requires $\vu{i}_B$ to be in the same vertical half plane as $\vu{h}$ {\color{red}This sentence is not clear.
% We can define a plane by every two non-parallel vectors.}. 
Figure \ref{fig:reference_frame} (b) shows a visual representation of constraints \eqref{eq:heading_constraint_1} and \eqref{eq:heading_constraint_2}. 
Assuming the quadcopter is not flipped over (i.e. $\vu{k}_B.\vu{k} > 0$), $\vu{i}_B$ and $\vu{j}_B$ are obtained by
% Assuming the quadcopter is not flipped over (i.e. $\vu{k}_B.\vu{k} > 0$), the heading constraints restrict $\vu{i}_B$ and $\vu{j}_B$ to:
% Given a local up-ward vector $\vu{k}_B$ and 
\begin{subequations}
\label{eq:base}
\begin{equation}
\label{eq:i_b}
    \vu{i}_B = \frac{\left(\vu{k} \times \vu{h}\right) \times \vu{k}_B}{\left|\left|\left(\vu{k} \times \vu{h}\right) \times \vu{k}_B\right|\right|}
\end{equation}
\begin{equation}
    \vu{j}_B  = \vu{k}_B \times \vu{i}_B
\end{equation}
\end{subequations}
{\color{red}Alternatively, yaw can be computed from $\vu{i}_B$ using:
\begin{equation}
\label{eq:atan}
    \psi = \atann\left(\vu{h}\cdot\vu{j}, \vu{h}\cdot\vu{i}\right),
\end{equation}
% \begin{equation}
% \label{eq:atan}
%     \psi = \atann\left(\vu{i}_B.\vu{j}, \vu{i}_B.\vu{i}\right),
% \end{equation}
where $\atann$ is the function which maps a 2d vector's y and x components to its principal angle \cite{atan2paper}. It has the property:
\begin{equation}
    \atann(A\sin(\theta), A\cos(\theta)) = \theta, \quad \forall \theta \in \left[-\pi, \pi\right], \forall A \in \mathbb{R}^{+}.
\end{equation}
}
% Note: The denominator in Eq. \eqref{eq:i_b} is zero only if the quadcopter is about to flip over.
% {\color{red}Alternatively, yaw can be computed from $\vu{i}_B$ using:
% \begin{equation}
% \label{eq:atan}
%     \psi = \atann\left(\vu{h}\cdot\vu{j}, \vu{h}\cdot\vu{i}\right),
% \end{equation}
% % \begin{equation}
% % \label{eq:atan}
% %     \psi = \atann\left(\vu{i}_B.\vu{j}, \vu{i}_B.\vu{i}\right),
% % \end{equation}
% where $\atann$ is the function which maps a 2d vector's y and x components to its principal angle \cite{atan2paper}. It has the property:
% \begin{equation}
%     \atann(A\sin(\theta), A\cos(\theta)) = \theta, \quad \forall \theta \in \left[-\pi, \pi\right], \forall A \in \mathbb{R}^{+}.
% \end{equation}
% }
\subsection{Differential flatness}
Using the heading constraint and the translation dynamics equation \eqref{eq:translation}, we can write angular velocity $\boldsymbol{\omega}$, thrust $p$, and their derivatives as algebraic functions of position $\boldsymbol{r}$, yaw angle $\psi$, and their derivatives. To this end, we express $\boldsymbol{\omega}$ and $\boldsymbol{\alpha}$ with respect to the body frame by
\begin{subequations}
\begin{equation}
    \boldsymbol{\omega} = \omega_x \vu{i}_B + \omega_y \vu{j}_B + \omega_z \vu{k}_B,
\end{equation}
\begin{equation}\label{alphaorginal}
    \boldsymbol{\alpha} = \alpha_x \vu{i}_B + \alpha_y \vu{j}_B + \alpha_z \vu{k}_B.
\end{equation}
\end{subequations}
By taking time-derivative from translational dynamics \eqref{eq:translation} and the first heading constraint equation \eqref{eq:heading_constraint_1}, we obtain $\dot{p}$, $\vb{h}_\omega=\boldsymbol{\omega} \times \vu{k}_B$, $\omega_x$, and $\omega_y$ by
\begin{subequations}
\label{eq:proj_1}
    \begin{equation}
        \dot{p} = m \dddot{\boldsymbol{r}}\cdot\vu{k}_B,
    \end{equation}
\begin{equation}
    \vb{h}_\omega = \frac{m \dddot{\boldsymbol{r}} - \dot{p}\vu{k}_B}{p},
\end{equation}
    \begin{equation}
        \omega_x = -\vb{h}_\omega\cdot\vu{j}_B,
    \end{equation}
    \begin{equation}
        \omega_y = \vb{h}_\omega.\vu{i}_B,
    \end{equation}
% \begin{equation}
% \label{eq:om_k}
%      \omega_k  = \frac{\omega_j \left(\vu{k} \times \vu{h}\right) .\vu{k}_B + \dot{\psi}\vu{h} . \vu{i}_B}{\left(\vu{k} \times \vu{h}\right) .\vu{j}_B}.
% \end{equation}
\end{subequations}
To obtain $\omega_z$, we express $\boldsymbol{\omega}$ as
$
\boldsymbol{\omega} = \dot{\phi} \vu{i}_B + \dot{\theta}  \left(\vu{k}\times \vu{h}\right) + \dot{\psi}\vu{k}
$, $\dot{\phi}=\omega_x$. Therefore, we can say
\begin{equation}\label{middleproof}
    \omega_y \vu{j}_B + \omega_z \vu{k}_B=\dot{\theta} \left(\vu{k}\times \vu{h}\right) + \dot{\psi}\vu{k}.
\end{equation}
Because $\dot{\theta}\vu{k}\cdot \left(\vu{k}\times \vu{h}\right)=0$, $\omega_z$ is obtained by
\begin{equation}
    \omega_z={\dot{\psi}-\omega_y\left(\vu{j}_B\cdot \vu{k}\right)\over \vu{k}_B\cdot \vu{k}}
\end{equation}
By taking the second time derivative  from Eq. \eqref{eq:translation} and defining
\begin{equation}
\begin{split}
    \vu{h}_p =& m \ddddot{\boldsymbol{r}} - p \left(\boldsymbol{\omega} \times \left(\boldsymbol{\omega} \times \vu{k}_B\right)\right) - 2\dot{p}\left(\boldsymbol{\omega} \times \vu{k}_B\right),\\
 =&p\alpha_y\vu{i}_B-p\alpha_x\vu{j}_B+\ddot{p}\vu{k}_B
\end{split}
\end{equation}
variables $\ddot{p}$, $\omega_x$, and $\omega_y$ are obtained by

\begin{subequations}
\label{eq:proj_2}
    \begin{equation}
        \ddot{p} = \vu{h}_p.\vu{k}_B,
    \end{equation}
    \begin{equation}
        \alpha_x = - {\vu{h}_p\cdot \vu{j}_B\over p},
    \end{equation}
    \begin{equation}
        \alpha_y =  {\vu{h}_p\cdot \vu{i}_B\over p}.
    \end{equation}
%     \begin{equation}
%         \vu{h}_\alpha = \frac{\vu{h}_p - \ddot{p}\vu{k}_B}{p},
%     \end{equation}
%     \begin{equation}
%         \alpha_i = -\vu{h}_\alpha.\vu{j}_B,
%     \end{equation}
%     \begin{equation}
%         \alpha_j = \vu{h}_\alpha.\vu{i}_B,
%     \end{equation}
% \begin{equation}
% \begin{split}
%     V = \left(\ddot{\psi}\vu{h}+\dot{\psi}^2\left(\vu{k} \times \vu{h}\right)\right) . \vu{i}_B + 2\dot{\psi}\vu{h} . \left(\boldsymbol{\omega} \times \vu{i}_B\right) \\- \left(\vu{k} \times \vu{h}\right).\left(\boldsymbol{\omega} \times \left(\boldsymbol{\omega} \times \vu{i}_B\right)\right),
%     \end{split}
% \end{equation}
% \begin{equation}
% \label{eq:al_k}
% \alpha_k = \frac{V + \alpha_j \left(\vu{k} \times \vu{h}\right) .\vu{k}_B}{\left(\vu{k} \times \vu{h}\right) .\vu{j}_B}.
% \end{equation}
\end{subequations}
Now, by applying the $3-2-1$ Euler angle standard, $\boldsymbol{\alpha}$ can be expressed as
\begin{equation}\label{middlealpha}
    \boldsymbol{\alpha} = \alpha_x \vu{i}_B +\ddot{\theta}(\vu{k}\times \vu{h}) +\ddot{\psi}\vu{k}-\omega_x\omega_y\vu{k}_B+\omega_x\omega_z\vu{j}_B-\dot{\theta}\dot{\psi}\vu{h},
\end{equation}
where $\alpha_x=\ddot{\phi}$. By equating the right-hand sides of Eqs. \eqref{alphaorginal} and \eqref{middlealpha}, we obtain
\begin{equation}\label{midproof2}
    \ddot{\theta}(\vu{k}\times \vu{h}) +\ddot{\psi}\vu{k}-\omega_x\omega_y\vu{k}_B+\omega_x\omega_z\vu{j}_B-\dot{\theta}\dot{\psi}\vu{h}=\alpha_y \vu{j}_B+\alpha_z \vu{k}_B.
\end{equation}
By obtaining dot product of $\vu{k}$ and both sides of Eq. \eqref{midproof2}, the first and last terms on the left-hand side of  Eq. \eqref{midproof2} vanish, and $\alpha_z$ is obtained by
\begin{equation}\label{midproof2}
    \alpha_z={\ddot{\psi}-\omega_x\omega_y\vu{k}_B\cdot \vu{k}+\omega_x\omega_z\vu{j}_B\cdot \vu{k}-\alpha_y \vu{j}_B\cdot \vu{k}\over \vu{k}_B\cdot \vu{k} }.
\end{equation}
\section{Individual Quadcopter Control}
\label{sec:controllers}

Both the snap controller and Mellinger controller are designed to allow quadcopters to track a trajectory position $\boldsymbol{r}_T$ and trajectory yaw $\psi_T$.

\subsection{Snap controller}

The snap controller is split into a position controller and a yaw controller which work in parallel. The position controller tries to achieve a snap $\ddddot{\boldsymbol{r}}$ determined by:
\begin{equation}
\begin{split}
    \ddddot{\boldsymbol{r}}_{des} = \ & - \boldsymbol{K}_1 \left(\dddot{\boldsymbol{r}} - \dddot{\boldsymbol{r}}_T\right) - \boldsymbol{K}_2 \left(\ddot{\boldsymbol{r}} - \ddot{\boldsymbol{r}}_T\right) \\ - & \boldsymbol{K}_3 \left(\dot{\boldsymbol{r}} - \dot{\boldsymbol{r}}_T\right) - \boldsymbol{K}_4 \left(\boldsymbol{r} - \boldsymbol{r}_T\right),
\end{split}
\end{equation}
where $\left(\boldsymbol{K}_1, \boldsymbol{K}_2, \boldsymbol{K}_3, \boldsymbol{K}_4\right)$ are position gain matrices. The yaw controller tries to achieve a second yaw derivative $\ddot{\psi}$ determined by:
\begin{equation}
    \ddot{\psi}_{des} = - K_5 \left(\dot{\psi} - \dot{\psi}_T\right) - K_6 \left(\psi - \psi_T\right).
\end{equation}
where $\left(K_5, K_6\right)$ are yaw gain scalars.

For this, the yaw controller needs the current $\psi$ and $\dot{\psi}$ of the quadcopter. These can be obtained using Eq. \eqref{eq:atan} and Eq. \eqref{eq:om_k}.

Once $\ddddot{\boldsymbol{r}}_{des}$ and $\ddot{\psi}_{des}$ are obtained, it maps them to desired rotor angular speeds through the following steps:
\begin{enumerate}
    \item Computing $\ddot{p}_{des}$ and $\boldsymbol{\alpha}_{des}$ using Eq. \eqref{eq:proj_2}.
    \item Computing desired thrust $p_{des}$ by integrating $\ddot{p}_{des}$ twice.
    \item Computing desired torque $\boldsymbol{\tau}_{des}$ using Eq. \eqref{eq:rotational}.
    \item Computing desired rotor speeds using Eq. \eqref{eq:rotors}.
\end{enumerate}

\subsection{Mellinger controller}

The Mellinger controller is split into a position controller and an attitude controller which are cascaded with the first's output given to the second.

The position controller tries to achieve a force determined by:
\begin{equation}
    \boldsymbol{F}_{des} = - \boldsymbol{K}_p \left(\dot{\boldsymbol{r}} - \dot{\boldsymbol{r}}_T\right) - \boldsymbol{K}_v \left(\boldsymbol{r} - \boldsymbol{r}_T\right) + mg\vu{k} + m\ddot{\boldsymbol{r}}_T,
\end{equation}
where $\boldsymbol{K}_p$ and $\boldsymbol{K}_v$ are positive definite gain matrices.

This force is projected onto the current local up-ward vector to get the desired thrust:
\begin{equation}
    p_{des} = \boldsymbol{F}_{des}.\vu{k}_B,
\end{equation}
and normalized to get the desired local up-ward vector:
\begin{equation}
    \vu{k}_{B,des} = \frac{\boldsymbol{F}_{des}}{\lVert\boldsymbol{F}_{des}\rVert}.
\end{equation}
Note: This assumes $\lVert\boldsymbol{F}_{des}\rVert \neq 0$.

$\vu{i}_{B,des}$ and $\vu{j}_{B,des}$, along with the desired rotation matrix $\boldsymbol{R}_{des}$ are found using Eq. \eqref{eq:base} to compute attitude error as defined by: 
\begin{equation}
    \boldsymbol{e}_R = \frac{1}{2}\left(\boldsymbol{R}_{des}^T\boldsymbol{R}-\boldsymbol{R}^T\boldsymbol{R}_{des}\right)^\vee,
\end{equation}
where $\square^\vee$ is the vee map which maps skew-symmetric matrices to vectors:
\begin{equation}
    \begin{bmatrix}0&a&b\\-a&0&c\\-b&-c&0\end{bmatrix}^\vee = \begin{bmatrix}-c\\b\\-a\end{bmatrix}, \qquad \forall (a,b,c)\in \mathbb{R}^3.
\end{equation}

The trajectory angular velocity $\boldsymbol{\omega}_T$ is found using \eqref{eq:proj_1} to compute angular velocity error as defined by:
\begin{equation}
    \boldsymbol{e}_{\omega} = \boldsymbol{\omega} - \boldsymbol{\omega}_T
\end{equation}

The attitude controller then tries to achieve a torque determined by:
\begin{equation}
    \boldsymbol{\tau}_{des} = -\boldsymbol{K}_R\boldsymbol{e}_R -\boldsymbol{K}_\omega \boldsymbol{e}_{\omega},
\end{equation}
where $\boldsymbol{K}_R$ and $\boldsymbol{K}_\omega$ are diagonal gain matrices.

Finally, $p_{des}$ and $\boldsymbol{\tau}_{des}$ are used to compute desired rotor speeds using Eq. \eqref{eq:rotors}.


\section{Snap and Mellinger Control Used by a Multi-Quadcopter System}
In this section, we consider a quadcopter team  applying ``mellinger'' and ``snap'' controllers to acquire a desired affine transformation in a decentralized fashion through local communication. We identify the quadcopters by set $\mathcal{V}=\left\{1,\cdots,N\right\}$ ($N$ is the total number of quadcopters). An $n$-dimensional affine transformation is defined as a leader-follower problem with leaders defined by set $\mathcal{V}_L=\left\{1,\cdots,n+1\right\}$ and follower defined by set $\mathcal{V}_F=\left\{n+2,\cdots,N\right\}$. The inter-agent communication among the quadcopters are defined by graph $\mathcal{G}\left(\mathcal{V},\mathcal{E}\right)$ with edge set $\mathcal{E}\subset \mathcal{V}\times \mathcal{V}$. Given edge set $\mathcal{E}$, set $\mathcal{N}_i=\left\{j:\left(j,i\right)\in \mathcal{N}\right\}$ defines the in-neighbors of quadcopter $i\in \mathcal{V}$. Because leaders move independently leaders have no in-neighbors, and thus, $\mathcal{N}_i=\emptyset$, if $i\in \mathcal{V}_L$. On the other hand, followers evolve through local communication, therefore, $\mathcal{N}_i\neq \emptyset$, if $i\in \mathcal{V}_F$.  The reference trajectory of quadcopter $i\in \mathcal{V}$ is defined by
\begin{equation}\label{affinetrajectory}
\mathbf{r}_{i,T}(t)=\begin{cases}
\mathbf{Q}(t,t_0)\mathbf{r}_{i}\left(t_0\right)+\mathbf{d}\left(t\right)&i\in \mathcal{V}_L\\
\sum_{j\in \mathcal{I}_i}w_{i,j}\mathbf{r}_j&i\in \mathcal{V}_F
\end{cases}
,\qquad t\geq t_0
\end{equation}
In \eqref{affinetrajectory} $\mathbf{Q}\in \mathbb{R}^{3\times 3}$ is the Jacobian matrix, $\mathbf{d}\in \mathbb{R}^{3\times 1}$ is the rigid-body displacement vector, and $w_{i,j}>0$ is a constant communication weight between follower $i$ and in-neighbor $j\in \mathcal{I}_i$, where 
\begin{equation}
    \sum_{j\in \mathcal{I}_i}w_{i,j}=1.
\end{equation}
To assure inter-agent collision avoidance, we first let $\delta$, $\epsilon$, and $d_{min}$ denote the controller error bound, quadcopter size, and minimum separation distance in the initail configuration of the MQS at initial time $t_0$. We then guarantee collision avoidance by using 
the  sufficient condition, provided in Ref. \cite{rastgoftar2021scalable},  and limiting the  eigenvalues of matrix $\mathbf{U}\left(t\right)=\left(\mathbf{Q}^T(t)\mathbf{Q}(2)\right)^{1\over 2}$, denoted by $\lambda_1(t)$, $\lambda_2(t)$, and $\lambda_3(t)$, to satisfy
\begin{equation}
    \lambda_{i}(t)\geq {2\left(\delta+\epsilon\right)\over d_{min}}.
\end{equation}
% $\lambda_{min}={\delta+\epsilo}$



% \begin{subequations}
%     \begin{equation}
%         m \ddot{\boldsymbol{r}} = p\vu{k}_B - mg\vu{k}_1
%     \end{equation}
%     \begin{equation}
%         m \dddot{\boldsymbol{r}} = \dot{p}\vu{k}_B +p(\omega \times \vu{k}_B)
%     \end{equation}
%     \begin{equation}
%         \dot{p} = m \dddot{\boldsymbol{r}}.\vu{k}_B
%     \end{equation}
%     \begin{equation}
%         \frac{m \dddot{\boldsymbol{r}} - \dot{p}\vu{k}_B}{p} =  -\omega_i \vu{j}_B + \omega_j \vu{i}_B
%     \end{equation}
%     \begin{equation}
%         \omega_i = -\frac{m \dddot{\boldsymbol{r}} - \dot{p}\vu{k}_B}{p}.\vu{j}_B
%     \end{equation}
%     \begin{equation}
%         \omega_j = \frac{m \dddot{\boldsymbol{r}} - \dot{p}\vu{k}_B}{p}.\vu{i}_B
%     \end{equation}
% \end{subequations}

% \begin{subequations}
% \begin{equation}
%   (\vu{k} \times \vu{h}).\vu{i}_B = 0.
% \end{equation}
% \begin{equation}
%     (\vu{k} \times\dot{\vu{h}}) . \vu{i}_B + (\vu{k} \times \vu{h}) . (\omega \times \vu{i}_B) = 0
% \end{equation}
% \begin{equation}
%     (\vu{k} \times \dot{\psi}(\vu{k} \times \vu{h})) . \vu{i}_B + (\vu{k} \times \vu{h}) . (-\omega_j \vu{k}_B + \omega_k \vu{j}_B) = 0
% \end{equation}
% \begin{equation}
%     -\dot{\psi}\vu{h} . \vu{i}_B -\omega_j (\vu{k} \times \vu{h}) .\vu{k}_B + \omega_k (\vu{k} \times \vu{h}) .\vu{j}_B = 0
% \end{equation}
% \begin{equation}
%      \omega_k  = \frac{\omega_j (\vu{k} \times \vu{h}) .\vu{k}_B + \dot{\psi}\vu{h} . \vu{i}_B}{(\vu{k} \times \vu{h}) .\vu{j}_B}
% \end{equation}
% \end{subequations}
% \
% \

% \

% \

% \

% \


% \
% \

% \

% \
% \

% \begin{subequations}
%     \begin{equation}
%         m \ddot{\boldsymbol{r}} = p\vu{k}_B - mg\vu{k}_1
%     \end{equation}
%     \begin{equation}
%         m \ddddot{\boldsymbol{r}} = \ddot{p}\vu{k}_B +2\dot{p}(\omega \times \vu{k}_B) + p(\alpha \times \vu{k}_B + (\omega \times (\omega \times \vu{k}_B)))
%     \end{equation}
%     \begin{equation}
%         \vu{h}_p = m \ddddot{\boldsymbol{r}} - p (\omega \times (\omega \times \vu{k}_B)) - 2\dot{p}(\omega \times \vu{k}_B)
%     \end{equation}
%     \begin{equation}
%         \ddot{p} = \vu{h}_p.\vu{k}_B
%     \end{equation}
%     \begin{equation}
%         \vu{h}_\alpha = \frac{\vu{h}_p - \ddot{p}\vu{k}_B}{p} =  -\alpha_i \vu{j}_B + \omega_j \vu{i}_B
%     \end{equation}
%     \begin{equation}
%         \alpha_i = -\vu{h}_\alpha.\vu{j}_B
%     \end{equation}
%     \begin{equation}
%         \alpha_j = \vu{h}_\alpha.\vu{i}_B
%     \end{equation}
% \end{subequations}

% \begin{subequations}
% \begin{equation}
%   (\vu{k} \times \vu{h}).\vu{i}_B = 0.
% \end{equation}
% \begin{equation}
% \begin{split}
%     (\vu{k} \times \ddot{\vu{h}}) . \vu{i}_B + 2(\vu{k} \times \dot{\vu{h}}) . (\omega \times \vu{i}_B) \\+ (\vu{k} \times \vu{h}) . (\alpha \times \vu{i}_B + \omega \times (\omega \times \vu{i}_B)) = 0
%     \end{split}
% \end{equation}
% \begin{equation}
% \begin{split}
%     A = -(\vu{k} \times \ddot{\vu{h}}) . \vu{i}_B - 2(\vu{k} \times \dot{\vu{h}}) . (\omega \times \vu{i}_B) \\- (\vu{k} \times \vu{h}) .(\omega \times (\omega \times \vu{i}_B)
%     \end{split}
% \end{equation}
% \begin{equation}
% (\vu{k} \times \vu{h}) . (\alpha \times \vu{i}_B) = A
% \end{equation}
% \begin{equation}
% (\vu{k} \times \vu{h}) . (-\alpha_j \vu{k}_B + \alpha_k \vu{j}_B) = A
% \end{equation}
% \begin{equation}
% -\alpha_j (\vu{k} \times \vu{h}) .\vu{k}_B + \alpha_k (\vu{k} \times \vu{h}) .\vu{j}_B = A
% \end{equation}
% \begin{equation}
% \alpha_k = \frac{A + \alpha_j (\vu{k} \times \vu{h}) .\vu{k}_B}{(\vu{k} \times \vu{h}) .\vu{j}_B}
% \end{equation}
% \end{subequations}


